Filtered Hyperbolic Moment Method for the Vlasov Equation

In this paper, we investigate the effect of the filter for the hyperbolic moment equations(HME) [15] of the Vlasov-Poisson equations and propose a novel quasi time-consistent filter to suppress the numerical recurrence effect. By taking properties of HME into consideration, the filter preserves a lot of physical properties of HME, including Galilean invariance and the conservation of mass, momentum and energy. We present two viewpoints, collisional viewpoint and dissipative viewpoint, to dissect the filter, and show that the filtered hyperbolic moment method can be treated as a solver of Vlasov equation. Numerical simulations of the linear Landau damping and two stream instability are tested to demonstrate the effectiveness of the filter in restraining recurrence arising from particle streaming. Both the analysis and the numerical results indicate that the filtered HME can capture the evolution of the Vlasov equation, even when phase mixing and filamentation are dominant.

==> article_todo.tex <==
\section{Conclusion}
In summary, ...
%the hyperbolic moment system has been derived for the 
%Vlasov-Maxwell equations. We have proven that the moment method conserves
%charge, conserves momentum, conserves energy and is stable. The corresponding
%numerical method is developing for the moment system obtained, and will be 
%apply to study important plasma physics problems in the future.
\begin{enumerate}
    \item 解释滤波器对电场能衰减速率和震荡频率的影响都很小
    \item $t>150$ 后，电场能大小为 $N \mu$，其中 $N$ 为网格数， $\mu$ 为机器精度。
        \item 说明滤波器不改变 Landau 阻尼电场能衰减率时。
            从三个角度说，
            首先说明在未出现 recurrence 之前和没有滤波器前的情况几乎一样；
            其次，
            说明出现之后，
            加入滤波器所得的衰减速率能和之前的结果几乎一样。
            最后说明在极限意义下，加入滤波器的结果和衰减速率的理论解可以一致。
            这个就涉及到矩数和网格剖分方向的收敛性了。
			\item $k=0.2,0.3,0.4$ 的情况还未计算。
			\item 对比未加 filter 和加入 filter 以后算的最好的参数。
			\item 未出现 recurrence 之前加不加 filter 的局部放大图。
			说明加入 filter 以后，没有出现 recurrence 时，
			和 HME 的结果几乎一样。
			\item 用图说明加密空间网格对于数值结果的影响并不大。
\end{enumerate}

\section*{Acknowledgements} This research of Y. Di is supported in
part by the Natural Science Foundation of China No. 11271358. 
%R. Li is supported in part by
%the National Basic Research Program of China (2011CB309704) and the
%National Natural Science Foundation of China No. 11325102 and No.
%91330205.


